Nonlinear Stability Analysis of Transitional Flows using Quadratic Constraints

The dynamics of transitional flows are governed by an interplay between the non-normal linear dynamics and quadratic nonlinearity in the incompressible Navier-Stokes equations. In this work, we propose a framework for nonlinear stability analysis that exploits the fact that nonlinear flow interactions are constrained by the physics encoded in the nonlinearity. In particular, we show that nonlinear stability analysis problems can be posed as convex feasibility and optimization problems based on Lyapunov matrix inequalities, and a set of quadratic constraints that represent the nonlinear flow physics. The proposed framework can be used to conduct global stability, local stability, and transient energy growth analysis. The approach is demonstrated on the low-dimensional Waleffe-Kim-Hamilton model of transition and sustained turbulence. Our analysis correctly determines the critical Reynolds number for global instability. For local stability analysis, we show that the framework can estimate the size of the region of attraction as well as the amplitude of the largest permissible perturbation such that all trajectories converge back to the equilibrium point. Additionally, we show that the framework can predict bounds on the maximum transient energy growth. Finally, we show that careful analysis of the multipliers used to enforce the quadratic constraints can be used to extract dominant nonlinear flow interactions that drive the dynamics and associated instabilities.

==> OptimalPert-Deleted.tex <==
\begin{comment}
\ak{
\section{Estimating Optimal Perturbations}
\label{sec:OptimalPert}

In this section, we show that the worst-case initial condition leading to MTEG---a so-called \emph{optimal perturbation}---can be obtained from the eigendecomposition of the Lyapunov energy matrix $P$ found from Eq.~\eqref{eq:Local_MTEGcalc_nonlinear}. Note that  $P$ defines the ellipsoidal set $S_R=\{\mathbf{x}: V(\mathbf{x})<R^2\}$, so the eigendecomposition of the $P$ provides essential information on the direction of largest and smallest gain. Since $P=P^T\succ 0$, without loss of generality, the eigenvalues can be ordered as $\lambda_{max}(P)\ge \cdots \ge \lambda_{min}(P)>0$, it follows that $\lambda_{min}(P) E(t) \le \mathbf{x}^TP\mathbf{x}\le \lambda_{max}(P)E(t)$. %where $\lambda_{max}(P)$ provides the scaling information and the eigenvector $v_{max}$ corresponding to $\lambda_{max}$ provides information on the direction of maximum energy growth. % here the eigenvalues $\lambda_{min}$ and $\lambda_{max}$ give us information on the scaling and their corresponding eigenvectors give the direction of minimum and maximum energy growth, respectively. 
As seen previously in Section~\ref{sec:QC_MTEG}, MTEG is upper bounded by $q$, more specifically, $\Theta \le q$. Here, $q$ is the magnitude of the energy growth and the eigendirection $\frac{v_{max}}{\|v_{max}\|}$ corresponding to $\lambda_{max}$ is the direction of maximum energy growth. Therefore, to identify the optimal perturbation, using the QC framework, we identify $\frac{v_{max}}{\|v_{max} \|}$ as the unit  direction vector of MTEG---obtained from an eigendecomposition of $P$---and we scale the perturbation's magnitude to lie on a sphere of radius $R_0=\frac{R}{\sqrt{q}}$. %It should be noted that MTEG is defined such that energy is lower bounded by unity and upper bounded by the condition number of $P$ i.e., $1\le \mathbf{x}^TP\mathbf{x} \le \frac{\lambda_{max}}{\lambda_{min}}$. More generally, to estimate the direction of largest energy growth, it follows that the energy growth is upper bounded by $\mathbf{x}^TP\mathbf{x} \le \lambda_{max}\mathbf{x}^T\mathbf{x}$, with equality resulting when $\mathbf{x}$ is in the eigendirection $\frac{v_{max}}{\|v_{max}\|}$ associated with $\lambda_{max}$. Therefore, the eigenvector $v_{max}$ corresponding to the largest eigenvalue $\lambda_{max}$ provides information on the direction of maximum amplification. %An initial condition on the largest permissible sphere of radius $R_0$ provides amplification in the direction of largest gain and hence causes MTEG. 
%More precisely, if the eigenvector associated with the largest eigenvalue is given by $v_{max}$, then the direction of largest possible growth is given by $\frac{v_{max}(P)}{\|v_{max}(P)\|}$. %Any random initial condition such that $\|\mathbf{x}_0\|=\frac{R}{\sqrt{q}}$, projected onto the normalized eigenvector $\frac{v_{max}(P)}{\|v_{max(P)}\|}$ will obtain the worst-case initial condition that causes the largest transient energy growth. 

%We compare the initial condition obtained from eigendecomposition of $P$, with that of the nonlinear optimal perturbation using the DAL. 
\sloppy The optimal perturbations obtained from the proposed framework are compared against the nonlinear optimal perturbations obtained using the DAL method~\citep{Kerswell2014,Kerswell2018}. 
%
%For both the methods, the optimal perturbations magnitude are scaled to lie on a sphere of radius $R_0 =\frac{R}{\sqrt{q}}$. 
We report magnitude and unit direction vector of the optimal perturbations from the two approaches to facilitate comparison of the results. %Here, we report optimal perturbations normalized to have a unit norm given by $\mathbf{x}_{0_{N}}=\frac{\mathbf{x}_{0_{opt}}}{\|\mathbf{x}_{0_{opt}} \|}$.
For the W parameter case, we obtain a magnitude $\|\mathbf{x}_{0_{opt}}^{QC}\| =\|\mathbf{x}_{0_{opt}}^{DAL}\|=R_0=6.8115\times 10^{-4}$, using $R=10^{-2}$ and its associated $q$ as shown in FIG.~\ref{fig:montecarlo}.  For this case of parameters, the optimal perturbation's unit direction vector as obtained from the QC framework and DAL method are $\frac{\mathbf{x}_{0_{opt}}^{QC}}{\|\mathbf{x}_{0_{opt}}^{QC}\|} =  \begin{bmatrix}-0.00023 & 0.99999 & 0.00000 & 0.00000 \end{bmatrix}^T$ and $\frac{\mathbf{x}_{0_{opt}}^{DAL}}{\| \mathbf{x}_{0_{opt}}^{DAL}\|} = \begin{bmatrix} 0.00826 & 0.99996 & 0.0000 & -0.00011 \end{bmatrix}^T$, respectively.
%
Similarly, for the B\&T parameters, we obtain a magnitude $\|\mathbf{x}_{0_{opt}}^{QC}\|=\|\mathbf{x}_{0_{opt}}^{DAL}\|=R_0=1.9965 \times 10^{-6}$, using $R=10^{-4}$ and its associated $q$ as shown in FIG.~\ref{fig:montecarlo}. In this case, the unit direction vectors of the optimal perturbation are $\frac{\mathbf{x}_{0_{opt}}^{QC}}{\|\mathbf{x}_{0_{opt}}^{QC} \|} =  \begin{bmatrix}0.00000 & 0.99999 & 0.00000 & 0.00000 \end{bmatrix}^T$ and $\frac{\mathbf{x}_{0_{opt}}^{DAL}}{\| \mathbf{x}_{0_{opt}}^{DAL}\|} = \begin{bmatrix} 0.00831 & 0.99996 & 0.00000 & 0.00000 \end{bmatrix}^T$. 

We use the inner product between the unit direction vector of the optimal perturbations to quantify their similarity.
%
If the optimal perturbations are closely aligned, then the inner product will be $\approx 1$. 
%
For the W parameters, the inner product yields $\langle \frac{\mathbf{x}_{0_{opt}}^{QC}}{\|\mathbf{x}_{0_{opt}}^{QC} \|},\frac{\mathbf{x}_{0_{opt}}^{DAL}}{\|\mathbf{x}_{0_{opt}}^{DAL}\|} \rangle = 0.999966$, indicating that the QC and DAL methods result in comparable optimal perturbations.
%
Similarly for the B\&T parameters we find that $\langle \frac{\mathbf{x}_{0_{opt}}^{QC}}{\|\mathbf{x}_{0_{opt}}^{QC}\|},\frac{\mathbf{x}_{0_{opt}}^{DAL}}{\| \mathbf{x}_{0_{opt}}^{DAL}\|} \rangle = 0.999965$, again confirming that the QC and DAL methods yield comparable optimal perturbations.
%It can also be verified that the optimal perturbations from the QC framework and DAL framework are aligned in the same direction i.e., they have a similar shape. Similar findings can also be observed for other parameter values. 

In addition to the optimal perturbations, the TEG response obtained from these perturbations are shown in FIG.\ref{fig:nonlinearWx0}. We show TEG response from an optimal perturbation computed from the eigendecomposition of P~(blue) and from DAL~(red). 
%In FIG.~\ref{fig:nonlinearWx0}, we show TEG obtained from the eigendecomposition of $P$ in blue and the TEG obtained from nonlinear optimal perturbation using the nonlinear DAL in red.
Additionally, we also show TEG from $1000$ Monte Carlo simulations in gray. The Monte Carlo simulations are obtained using random initial conditions sampled from a sphere of radius $R_0 =\frac{R}{\sqrt{q}}$. %For the W parameters, we use $R=10^{-2}$ and its associated MTEG bound~($q$) to obtain $\|\mathbf{x}_{0_{opt}}^{QC}\|=6.8115\times 10^{-4}$. In the B\&T parameter case we use $R=10^{-4}$ and its associated MTEG bound~($q$) to obtain an initial condition $\|\mathbf{x}_{0_{opt}}^{QC}\|=1.99\times 10^{-6}$. These $R$ and $q$ values are taken from the results reported in FIG.~\ref{fig:montecarlo}.
}
\end{comment}
\begin{comment}
\begin{table}[!htb]
\centering
    \begin{tabular}{|c|c|c|}
    \hline
   Parameter set  & \multicolumn{2}{|c|}{Optimal Perturbation}\\\cline{2-3}
   \hline\hline
         & QC & DAL   \\
        \hline
         W~\citep{WaleffePOF1995}& $\begin{bmatrix}-3 & 9 & 0& 0\end{bmatrix}$^T & \\
         \hline
         B\&T~\cite{BaggetPOF1997} & & \\
         \hline
    \end{tabular}
    \caption{Comparison of the normalized optimal perturbation from QC framework and DAL.}
    \label{table:1}
    \end{table}


\begin{figure}[!htb]
    \centering
    \subfloat[W parameters, $Re=250$]{\includegraphics[scale=0.4]{../PRFluids-Rebuttal/RebuttalPlots/Wx0/WKH_PRFParamsRe250_MonteCarlo1e3_PertSize6.81e-4_NonLinWx0VsQC_v2.png}}
    \subfloat[B\&T parameters, $Re=100$]{\includegraphics[scale=0.4]{../PRFluids-Rebuttal/RebuttalPlots/Wx0/WKH_BTParams_MonteCarlo1e3_R1.99e-6_NonLinWx0VsQCWx0.png}}
    \caption{TEG response from nonlinear optimal perturbation obtained from QC framework, DAL, and Monte Carlo simulations.}
    \label{fig:nonlinearWx0}
\end{figure}
\end{comment}

==> R0_Analysis2.tex <==
\section{Estimating Permissible Perturbation Amplitudes}
\label{sec:stabilityBoundary}

We have shown that the GEVP in Eq.~\eqref{eq:GEVP_ROA} can be solved to obtain the largest lower bound on $R$. Now we aim to identify the largest perturbation size $R_0$, such that trajectories originating in a sphere of radius $R_0$ will converge back to the equilibrium. The sphere of radius $R_0$ is obtained by finding the largest inner approximation of the ROA---this sphere is a sub-level set of the ellipsoid  $V(\mathbf{x}) \le R^2$. The size and shape of the ellipsoid depends on the energy weight matrix $P$ found in Eq.~\eqref{eq:GEVP_ROA}.
We will show that the GEVP can be used to estimate the largest perturbation amplitude $R_0$ that drives the trajectory to the edge of stability.% (i.e., the minimal seed~\citep{Pringle2012}).

Consider initial conditions inside a sphere of radius $R_0$ around the equilibrium point such that $||\mathbf{x}_0||^2 \le R_0^2$.  Let $q:=\lambda_{max}(P)/\lambda_{min}(P)$ be the condition number of $P$ with $\lambda_{max}$ and $\lambda_{min}$ being the largest and smallest eigenvalues of $P$, respectively. The condition number $q$ of  matrix $P$ provides information on the skewness of the bounding ellipsoid. To bound the skewness of the elliptical set, we can simply bound $P$ as $I \preceq P \preceq qI$. We now seek to determine the largest sphere of initial conditions $\|\mathbf{x}_0\|^2 \le R_0^2$ such that trajectories remain inside the ROA. %The Lyapunov function is upper bounded by $R$ i an invariant set $S_r = \{\mathbf{x}: V(\mathbf{x})<R^2\}$ (see Appendix~\ref{sec:appendixA} for proof). %In Appendix~\ref{sec:appendixA}, we show that if $V(\mv{x}(0))<R^2$ then the set $S_r=\{x \in \R^n|V(\mv{x})<R^2 \}$ is the ROA. Given $S_r$ is the ROA, we analyze the  maximum allowable radius of sphere $R_0$ for initial perturbation such that $\|\mathbf{x}_0\|^2 \le R_0^2$ and the trajectories always remain in the invariant set $S_r$. 
From the inequality $I\preceq P\preceq qI$ and $\dot{V}(\mathbf{x})<0$, it follows that
    $\|\mv{x}\|^2 \le \mv{x}^TP\mv{x} \le \mv{x}_0^TP\mv{x}_0 \le q\|\mv{x}_0\|^2$, which implies that $\|\mv{x}\|^2 \le q\|\mv{x}_0\|^2$. Therefore, we have $\|\mv{x}\|^2 \le {qR_0^2}={R^2}$, 
and we can find the largest allowable sphere of radius $R_0$. To do so,
we can now use the decomposition of $M_i=R^2\tilde{M}_i+\hat{M}_i$ (see Eq.~\eqref{eq:Mdecomposition}) and the relation $R^2=qR_0^2$, then solve the following GEVP 
	
	\begin{align}
	\begin{split}
	\text{minimize} \quad & t_0\\
	\mbox{subject to}~& I\preceq P\preceq qI\\
	& \xi_{p_i} \ge 0 \qquad (\text{for i=1 to 4})\\
	&  \begin{bmatrix} A^TP + PA & P\\
	P & \mv{0}\end{bmatrix} + \xi_{p_0}M_0 + \sum_{i=1}^4 \xi_{p_i}\hat{M}_i \prec t_0 q \sum_{i=1}^4 \xi_{p_i}\tilde{M}_i,
	\label{eq:GEVPR0}
	\end{split}
	\end{align}
  where $t_0=-R_0^2$.  To solve for the largest permissible perturbation amplitude, we solve Eq.~\eqref{eq:GEVPR0} over a grid of $q$ values, then pick the solution corresponding to the largest $R_0$.
	
We verify our findings by comparing the $R_0$ obtained from the proposed quadratic constraints~(QC) framework with the nonlinear optimal perturbations obtained using nonlinear direct-adjoint looping~(DAL), as detailed in \citep{Kerswell2014,Kerswell2018}. In the DAL method, a so-called ``minimal seed'' is obtained using the calculus of variations and a gradient method to find the nonlinear optimal perturbation on a sphere of radius $R_0$. If divergent trajectories are found for perturbations of size $R_0$, we update the upper and lower bounds on $R_0$ via bisection. Once the upper and lower bounds converge to some tolerance $\epsilon > 0$ (here $\epsilon = 10^{-8}$) and no divergent trajectories are found, we terminate the bisection procedure. Since DAL uses the exact nonlinear equations of motion, it provides accurate estimates for the minimal seed of the nonlinear system and the permissible amplitude. In addition to the DAL method, we also compare with results from the sum-of-squares~(SOS) framework using quadratic energy functions~\citep{goulart2012}. Both the SOS and QC framework use Lyapunov-based methods to compute the largest sphere of radius $R_0$, which is an inner approximation of the ROA, and hence these methods are conservative in their estimates of the permissible perturbation amplitude.

In FIG.~\ref{fig:R0plot}, we report the largest radius of initial conditions $R_0^*$ versus $Re$ using the three methods mentioned above. For the B\&T parameters we show results of the DAL~($\triangle$), SOS framework~($\square$), and QC framework~($\bigcirc$) in FIG.~\ref{fig:BT_R0}. However, for the W parameters we compare the results of the SOS framework and QC framework only in FIG.~\ref{fig:W_R0}, this is because for the W parameters no divergent trajectories were found using DAL. Even though there are no divergent trajectories the SOS framework and QC framework provide conservative estimates for $R_0$, as expected.
%The overall prediction by the QC framework can be considered as conservative as seen in FIG.~\ref{fig:R0plot}. It can be seen that the DAL and SOS framework are relatively close to each other in their prediction of the largest $R_0$ in FIG.~\ref{fig:BT_R0}, this is predominantly because SOS framework uses the information of the ``exact'' nonlinear term to make predictions while the DAL method also uses nonlinear simulations that account for the nonlinear terms exact behavior. Meanwhile the QC framework uses constraints to capture the behavior of the nonlinear terms, hence adding further constraints to this framework will reduce the conservativeism  of the results.
\begin{figure}[!htb]
    \centering
    \subfloat[W parameters]{\includegraphics[scale=0.5]{WKH_PRFParameters_GEVPVsSOSVsDAL_New.eps}
    \label{fig:W_R0}}
   \subfloat[B\&T parameters]{\includegraphics[scale=0.5]{WKH_BTParameters_GEVPVsSOSVsDAL_New.eps}\label{fig:BT_R0}}
    \caption{The maximum allowable perturbation size $R_0$ as a function of $Re$ for W and B\&T parameters compared against the SOS framework and DAL method.}
    \label{fig:R0plot}
\end{figure}

For the  B\&T parameters, the largest allowable perturbation size for $Re=100$ is found to be $R_0^*\approx 1.5 \times 10^{-5}$ using the QC framework; this is a conservative estimate relative to $R_0^*=10^{-4}$ in~\citep{BaggetPOF1997}. As seen in both figures in FIG.~\ref{fig:R0plot}, we observe that the $R_0^*$ predicted by the QC framework is conservative. Since the QC framework does not use detailed information of the nonlinear terms---it only uses a few constraints that characterize the input-output behavior of the nonlinear terms---this behavior is expected.  In exchange for this conservatism, the QC framework is less computationally expensive compared to the SOS and DAL methods, which are more computationally expensive and may not be suitable for large systems. %Another reason for the conservative estimates in this method is due to the formulation of the problem in Eq.~\eqref{eq:feasibility_lmi}. Since, we are not directly solving an optimization problem that maximizes $R_0$ and instead we are bisecting over various $R$ to obtain the largest feasible $R_0$, we expect our results to be more conservative. 
We finally note that recent works by Liu and Gayme~\citep{Liu2020}---which appeared during the review of this manuscript---have aimed to reduce conservatism of these estimates within the QC framework.%shown an alternative formulation for the minimal seed problem using a similar QC framework, their approach is aimed at reducing this conservatism.

==> intro.tex <==
\subsection{Motivation and Problem Statement}

In this paper, we propose a constrained nonlinear systems analysis approach that 
generalizes established linear stability and input-output analysis techniques to account for nonlinear 
flow interactions.  The approach is predicated on the fact that nonlinear flow interactions are 
constrained by the physics encoded within the nonlinear terms in the Navier-Stokes equations~(NSE).
Mathematically, these physics can be expressed as quadratic constraints between the 
inputs and outputs of the nonlinearity.  In turn, these quadratic constraints enable a reduced-complexity modeling of nonlinear terms, and can be incorporated within a Lyapunov-based analysis to  perform reliable stability and input-output analysis in the nonlinear setting. 

In wall bounded shear flows, the NSE can be partitioned into a non-normal linear block acting in feedback with a static lossless nonlinear block---called the Lur\'e system (see FIG.~\ref{fig:Lure_WKH}). The framework proposed here accounts for both the non-normal linear block and nonlinear block while investigating the systems stability and energy amplification~(performance).

In most fluid flow analysis, the nonlinear interactions of the NSE are not accounted for, since, a framework to efficiently account for specific structured nonlinear interactions does not exist. The general framework we propose can perform stability, performance and input-output analysis on any system that has a non-normal linear block acting in feedback with a static lossless nonlinearity---NSE being a special case for such a system. In general the linear systems stability and performance analysis problems can be investigated using Lyapunov analysis formulated as linear matrix inequalities~(LMI). Given a Lur\'e system, the linear systems LMI problem can be augmented by the addition of the aforementioned quadratic constraints---to account for  the effects of the nonlinear block. Therefore, we propose a general framework to enable reduced-complexity nonlinear stability, performance and input-output analysis of fluid flows. 


\subsection{Background}
Traditional hydrodynamic stability analysis rely on linearization of  the NSE equation around a base flow. Linear stability analysis often over predicts stability regimes, more so in wall-bounded shear flows~\citep{PatelJFM1969,ReddyJFM1993,Schmid2001}. These linear analysis methods have provided many powerful tools for analysis of fluid flows like global stability analysis~\citep{Theofilis2011}, adjoint-stability analysis~\citep{Luchini2014}, non-modal stability analysis~\citep{Schmid2001,Schmid2007}, etc. As observed in non-modal stability analysis, whereby non-normal linear dynamics results in transient energy growth~(TEG) of small-perturbations, TEG is a necessary condition to trigger a change in systems stability~(transition)~\citep{Trefethen1993,Schmid2007,HenningsonPOFComment}.
%Transition to turbulence negatively impacts many engineering systems~(e.g. airplanes, ships, wind turbines, etc.) as it deteriorates their operating efficiency by increasing skin-friction drag. Many efforts have sought to better understand and predict transition especially in shear flows~\citep{Schmid2007,HenningsonPOF1994,Chapman2002,Trefethen1993}. However, transition is a complex process involving the interplay between linear and nonlinear terms in the Navier-Stokes equations~(NSE). Hydrodynamic stability analysis of various shear flows has mostly relied on linear stability analysis by ignoring nonlinear terms; and it over predicts a critical Reynolds number ($Re_c$) for the on-set of turbulence~\citep{PatelJFM1969,ReddyJFM1993,Schmid2001}.  Research in transitional shear flows has greatly benefited from non-modal stability analysis, whereby non-normal linear dynamics results in transient amplification of small perturbations. The transient energy growth~(TEG) from these linear dynamics is a necessary condition for sub-critical transition~\citep{Trefethen1993,Schmid2007,HenningsonPOFComment}.
%These stability analysis rely on linearization of the nonlinear NSE to predict a critical Reynolds number~($Re_c$), below which all perturbations will decay. 
%In wall-bounded shear flows, laminar to turbulent transition has been observed to occur well below the $Re_c$ determined from linear stability analysis}. Since wall-bounded turbulent flows exhibit markedly greater skin-friction drag than laminar flows, the exact mechanisms responsible for transition have been of great research interest~\citep{Schmid2007,HenningsonPOF1994,Chapman2002,Trefethen1993}.
%
%Many works attribute the cause of sub-critical transition to a linear non-modal mechanism for transient energy growth~(TEG). 
%Much work in systems analysis and controller design in fluid mechanics has focused on the non-modal mechanisms in the linearized NSE,
%without explicitly accounting for the nonlinear interaction terms~\citep{Trefethen1993,MartinelliPOF2011,Kalur2018,Kalur2019,JovanovicJFM2005,KimAnnRev2006}. 
In spatially periodic flows, the linearized NSE consider infinitesimal perturbations, these perturbations are assumed to evolve independently at different wavelengths, however, in the nonlinear governing equations there is an interaction between disturbances at various wavelengths.

%--------------------
%These linear analysis methods have provided many powerful tools for analysis of fluid flows like global stability analysis~\citep{Theofilis2011}, Adjoint-stability analysis~\citep{Luchini2014}, Non-modal stability analysis~\citep{Schmid2001,Schmid2007}, etc.
%The dominance of linear terms in the energy-growth equations of Reynolds-Orr enables the exclusion of nonlinear terms in the sub-critical transition analysis and controller design process~\citep{Schmid2001,HenningsonPOFComment}; thereby making it a practical, realistic and effective approximation. The high-degree of non-normality of the linearized NSE operator results in a transient amplification of small perturbations, even when the dynamics are linearly asymptotically stable. 
%---------------------
The TEG of small perturbations interact with nonlinearities and can trigger secondary instabilities, leading to by-pass transition\citep{ReddyJFM1993}. % In wall-bounded shear flows, the linear dynamics interact with the nonlinearity in a feedback mechanism, and the NSE can be partitioned as a Lur\'e decomposition~\citep{Heins2016}. 
The exact interplay between non-normality and nonlinearity in the transition process is not fully understood.
%
However, it is well accepted that the linear terms in NSE contribute to the non-modal growth, whereas
the nonlinear terms contribute to mixing and vortex regeneration~\citep{BaggetPOF1997}.  Even though a linear systems approach works well for stability analysis and more so for control~\citep{KimAnnRev2006,Bewley2001}, it is necessary to account for the complex nonlinear interactions in the flow---to further enhance both our analysis and controller performance capabilities in fluid flow systems. %The linear and nonlinear elements interact with each other in a feedback mechanism.
%-------------------
% The linear and nonlinear terms in the WKH model are in a feedback interaction with each other. 
%The properties of linear and nonlinear elements in the NSE are leveraged to obtain low-dimensional models for understanding sub-critical transition. In~\citep{BaggetPOF1997}, the authors review several low-dimensional models that mimic the behaviour of NSE. Similarly, Waleffe develops low-dimensional models that mimic transition behavior of NSE in shear flows.
%
%In~\citep{WaleffeSIAM1995}, Waleffe highlights the importance of both the nonlinearity and non-normality in
%the transition process and for sustained turbulence.
%
%He introduces a low-dimensional non-linear model that mimics the behaviour of the NSE by capturing
%physical mechanisms central to the transition process.
%
%The low-dimensional Waleffe-Kim-Hamilton~(WKH) model consists of a non-normal linear element and
%a lossless nonlinearity similar to that in NSE.
%-------------------
%The mechanism for transition is complicated to understand due to interplay between complex nonlinear interactions.

%Frameworks for analyzing a linear element with nonlinearities and/or uncertainties acting in feedback
%have been well established in the robust-control community.
%Transition can be viewed as an issue in system robustness rather than system stability~\citep{GaymeThesis}.
%
%The large amplification of disturbances and changes in spectra based on the $\epsilon$-pseudospectral
%interpretation~\citep{Trefethen2005} extend themselves directly to system robustness issues.
%
%Therefore a robust control approach to study transition can account for both the linear and nonlinear terms in the NSE. Partitioning the feedback interconnection into two positive operators---the Lur\`e decomposition---is a standard approach in robust control theory and is often advocated for nonlinear system analysis.
\subsection{Previous works}
%
Recent efforts in literature have successfully attempted to account for the nonlinear interactions using frameworks such as resolvent analysis~\citep{McKeonJFM2010}. %, passivity ~\citep{Heins2016,Damaren2016,Damaren2018} and dissipation inequality~\citep{Ahmadi2018}.
The resolvent analysis framework leverages the feedback interaction between the linear and nonlinear operator in the NSE, by considering the nonlinear term as an implicit forcing input to the linear dynamics~\citep{McKeonJFM2010,TairaModal2017,Taira2019}. Resolvent analysis has been successfully employed in various contexts, namely identification of coherent structures in wall-turbulence in pipes~\citep{SharmaJFM2013}, identification of triadic nonlinear interaction between resolvent modes~\citep{MckeonAndSharmaPoF2014}, obtaining insights into compressible open cavity flows~\citep{Sun2019}, and passive flow control using riblets~\citep{Chavarin2019}. The resolvent analysis is an input-output framework, which provides information on how fluctuations in a time-averaged flow are attenuated or amplified from nonlinear effects. However, the resolvent framework does not explicitly account for the structure of the nonlinearity. %However, it is essential to note the resolvent operators requires only the linear term, the nonlinear term is assumed to implicitly force the resolvent operator to obtain desired output. 
Additionally, the passivity framework~\citep{Khalil} accounts for structure in the nonlinear terms---leveraging the passivity observed in the nonlinearity of the NSE. The passivity framework~\citep{Heins2016,Damaren2016,Damaren2018} has been shown to be effective in control applications for nonlinear NSE. %In~\citep{Heins2016,Damaren2016,Damaren2018}, passivity-based control methods for turbulent flows are proposed.  These methods rely on the passivity of the nonlinear terms in the NSE. Here a output feedback controller is developed to force the linear dynamics to be passive, without fully accounting for the exact nonlinearity. 
In both the resolvent and passivity analysis framework the nonlinear term is not explicitly accounted for.
%

Further advances have been made in input-output methods to study performance, worst-case amplification and transition for NSE using dissipation inequalities. In \citep{Ahmadi2018}, the dissipation inequalities framework is reformulated for the NSE. The authors pose the dissipation inequalities as matrix inequality problems, which are then solved using convex optimizations methods to successfully analyze the input-output performances in various wall-bounded flows. Alternatively, a wide range of analysis techniques have been proposed to assess the stability of fluid flows: e.g.,~modal and non-modal stability analysis~\cite{Theofilis2011, Schmid2007,McKeonJFM2010,TairaModal2017,Taira2019,Kerswell2018} as well as more recent undertakings that generalize the classical energy-based analysis approach~\cite{Schmid2001,josephBook} with Lyapunov analysis~\cite{goulart2012}. While the community has made significant progress in stability analysis and prediction, the most reliable of the existing analysis approaches still tend to provide conservative estimates for transition thresholds~\cite{Ahmadi2018}.

%Another input-output method is
%A Lur\'e decomposition of NSE  has also been for used for analysis and control within fluid mechanics community.
%Leveraging the Lur\'e decomposition, the passivity framework~\citep{Khalil} is used to develop 
%Here the passive property of the nonlinear term along with exact knowledge of the linear term in NSE is used for 

%In~\citep{Heins2016}, given the passive nonlinear term in turbulent channel flows, the authors control the linear dynamics with output feedback to demonstrate a reduction in skin-friction drag. Similarly, in~\citep{Damaren2016,Damaren2018}, Damaren uses passivity-based output control of laminar-turbulent transition on both the Orr-Sommerfeld Equation and Blasius boundary layer problem respectively. 
%Another approach to account for nonlinearity in NSE is shown in \citep{Ahmadi2018}. The authors introduce an input-output analysis framework using nonlinear partial differential equations~(PDEs) in wall-bounded shear flows. In \citep{Ahmadi2018}, the dissipation inequalities framework introduced by Willems~\citep{Willems1972}, is reformulated for nonlinear PDEs like the NSE. The authors pose the dissipation inequalities as matrix inequality problems, which are then solved using convex optimizations methods to successfully analyze the input-output performances in various wall-bounded flows. 


% ; extensive
% DNS and experimental campaigns are still required to more reliably determine the stability and
% transition characteristics of various flows.
%\subsection{Current work}

%\msh{MSH: this paragraph can be integrated within the one above.  Needs to be made more concise and pointed.} To develop insights into nonlinear stability and performance analysis, we need a framework that can reliably capture effects of the nonlinear interactions in transition, and also facilitate uncovering of underlying physics directly from the governing equations. 
%The general approach framework will be established by enabling a reduced-complexity representation of nonlinear interactions using quadratic constraints. The quadratic constraints are a collection of input-output constraints that quantify the behavior of the nonlinear terms in the system. 
%In general the linear systems stability and performance analysis problems can be investigated using Lyapunov analysis formulated as linear matrix inequalities~(LMI). Given a Lur\'e decomposition with linear and nonlinear blocks in feedback, the linear systems LMI problem can be augmented by the addition of the aforementioned quadratic constraints---to account for  the effects of the nonlinear block.  %Here, we treat the nonlinear element as a ``black-box'' and use quadratic constraints to quantify its input-output behavior.
\subsection{Current work}
We propose a method that unifies previously discussed stability, performance and input-output analysis methods into one framework that accounts for structure and physics observed in the nonlinear terms, by representing nonlinear behavior via quadratic constraints. The addition of these quadratic constraints to the linear system analysis problem facilitates nonlinear analysis without explicitly knowing the ``exact'' nonlinear terms. Once LMI's with constraints are formulated, convex optimization is used to search over combinations of these constraints to find one that provides the most accurate estimate of specified performance criteria. Quadratic constraints are used to assess the impact of nonlinearities and uncertainties on dynamical systems. As such, the quadratic constraints framework will do no worse than any of above listed existing methods, but can be tailored to the specific problem at hand---by  imposing additional constraints to describe the nonlinearity---in order to extract more reliable and precise predictions of transition.  
%the nonlinear blocks effect on the linear system can be captured by accounting for the input-output behavior of the nonlinear terms alone, without accounting for the exact nonlinearity. These input-output properties are represented using quadratic constraints.  With an accurate representation of the linear systems, and the nonlinear terms behavior are defined by quadratic constraints, 
% Now convex optimization is used to search over combinations of these constraints to find one that provides the most accurate estimate of specified performance criteria. Quadratic constraints are used to assess the impact of nonlinearities and uncertainties on dynamical systems. As such, the quadratic constraints framework will do no worse than any of above listed existing methods, but can be tailored to the specific problem at hand---by  imposing additional constraints to describe the nonlinearity---in order to extract more reliable and precise predictions of transition.  

In this paper, we introduce a quadratic constraints framework for accommodating nonlinear effects for reduced-complexity stability and transient energy growth analyses. %The quadratic constraints framework broadly combines concepts from input-output theory, absolute stability theory, and robust controls into a unifying framework~\citep{MegretskiIEEE1997}. 
%\msh{MSH: This paragraph can be made more concise. It will also be good to include a summary of all the findings (see bullets below for a start).}.
To establish a proof of concept, we demonstrate the proposed quadratic constraints-based  frameworks utility on the nonlinear Waleffe-Kim-Hamilton~(WKH) model, the WKH model is a low-dimensional model that captures mechanics of transition in shear flows~\citep{WaleffeSIAM1995}. Similar to the NSE, we first express the WKH system in Lur\'e form---a non-normal linear element in feedback interaction with a static lossless nonlinear element. Here, we formulate several quadratic constraints and investigate the role of the nonlinear terms for stability and transient energy growth analysis within the WKH model. In addition to passivity of the nonlinear term, the nonlinearity in wall-bounded shear flows has a stronger property of being lossless or energy conservation, which can be leveraged. Since the WKH model is developed to mimic the NSE's behavior in shear flows, the nonlinear terms in the WKH model are energy conserving as well. 
%
%
%
%, with non-normal linear dynamics in feedback with a static lossless nonlinearity.
%
The ``global'' energy-conserving property of the nonlinearity in the WKH model can be expressed in terms of a quadratic constraint between its inputs and outputs.
%
This quadratic constraint is then used to capture the influence of the nonlinearity on the linear dynamics, which is exploited for analyzing global stability and maximum transient energy growth~(MTEG) performance. Another aspect of this analysis is to investigate stability and MTEG of the system in a small region around the equilibrium, this is especially helpful in developing insights into transition and stability thresholds. Therefore, 
%
following the global analysis, we further extend the quadratic constraints framework to capture the nonlinear terms input-output behavior around a small neighbourhood of a given equilibrium point. The encoded local properties of the nonlinearity are represented as ``local'' constraints and this representation enables ``local'' stability and ``local'' MTEG analysis of the WKH system around a given equilibrium point. This analysis framework is not restricted to the WKH model, it is more general and will translate to any system having a linear and static nonlinear element in feedback, especially the NSE. 
%He introduces a low-dimensional non-linear model that mimics the behaviour of the NSE by capturing
%physical mechanisms central to the transition process.


%It should be noted that quadratic constraints framework can also be used for time-varying nonlinearities like in the the NSE. For time-varying nonlinearities we can extend the quadratic constraints framework to integral quadratic constraints~(IQCs)---capture nonlinear terms behavior between two time instances by integrating the constraints over time. The use of IQCs
%dates back to the work by Yakubovich~\citep{Yakubovich1971} and a general framework was given in~\citep{MegretskiIEEE1997}. Even though we develop the quadratic constraints framework on the nonlinear WKH system; this approach can also be applied to NSE directly using IQCs.
%
%I%QCs provide a general framework for stability and performance analysis, the IQCs are a powerful framework of which passivity and dissipativity frameworks are special cases.
%
The contributions of this work are:
%\msh{
%\begin{itemize}
   % \item Global stability Analysis: 
 \begin{enumerate}

    \item This work extends the linear system analysis methods by accounting for the nonlinear terms in the system. The energy conserving nonlinearity in the WKH system is accounted for via the addition of a quadratic lossless constraint. The lossless constraint alone enables prediction of the critical Reynolds number for global instability in the WKH system. This finding is consistent with the findings reported in Waleffe~\citep{WaleffePOF1995}.
    %\item Local stability Analysis: 
    
    \item Beyond the global stability regime in the WKH system, the quadratic constraint framework is extended to represent ``local'' nonlinear properties as ``local'' quadratic constraints---for analyzing stability of the nonlinear system in a local neighborhood of a given equilibrium point. These ``local'' constraints extend the stability and MTEG analyses to Reynolds numbers beyond the critical Reynolds number for global instability.  By modifying the size of the local region, the influence of the nonlinearity can be assessed. Given that the linear system is asymptotically stable for all $Re$, we show that the nonlinear term has a destabilizing effect on the system.
    
    %\item Maximum transient energy growth analysis: 
    \item Additionally, it is shown that the lossless and local constraints serves to enhance MTEG in the non-normal and nonlinear WKH system, consistent with findings from nonlinear non-modal stability analysis~\cite{Kerswell2018}.  Indeed, these findings confirm that the optimal disturbance for the nonlinear system is different from the linear optimal disturbance that is often used to study transient energy growth and transition.
    
    %\item Additional constraints can be introduced to constrain the flow state to remain within a local region of the equilibrium point.  These ``local'' constraints extend the stability and TEG analyses to Reynolds numbers beyond the critical Reynolds number for global instability.  By modifying the size of the local region, the influence of the nonlinearity can be assessed.  (state something about the results.)
    %\item 
    \item Lastly, when multiple constraints are included in the analysis, it becomes possible to identify dominant nonlinear flow interactions by analyzing the multipliers used to enforce the constraints within the analysis.  It is demonstrated that---without any a priori knowledge---the proposed analysis approach is able to extract the same dominant nonlinear flow interactions whose physical importance is argued in~\citep{WaleffePOF1995,WaleffeSIAM1995}.
%\end{itemize}
 \end{enumerate}
%These bullets can be integrated with the paper organization outline below.  This would make it more useful, since it would be a summary of results.  No need to start sentences with ``In Section...", but can ends sentences with ``\dots, as will be shown in Section\dots'' instead.
%}
%\ak{Note to self: try combining contributions and organization into 1 section?}
%
This paper is organized as follows: Section~\ref{sec:WKH} introduces the fluid flow model used in our analysis. In Section~\ref{sec:QC_stability}, we briefly describe the global property of the nonlinear terms in the WKH model and also introduce the quadratic constraints framework for both global and local stability, while also discussing stability results. In Section~\ref{sec:QC_MTEG}, we formulate quadratic constraints framework for both global and local MTEG analysis.  This sections also discuss the results obtained from local MTEG analysis. In Section~\ref{sec:Lagrange_Mul_Analysis}, we discuss how the quadratic constraint framework can be used to draw physical insights regarding dominating nonlinear flow interactions using Lagrange multiplier analysis. Finally, we provide the concluding remarks of our study in Section~\ref{sec:Conclusion}.

==> intro2.tex <==
Many complex flow phenomena arise from the interplay 
between non-normal linear dynamics and a quadratic 
nonlinearity in the Navier-Stokes equations~(NSE).
%
It is well-established that the linear dynamics
drive non-modal mechanisms for transient energy growth~(TEG)~\citep{schmid2001,schmid2007,Trefethen1993}.
%
The high-degree of non-normality of the linear(ized) NSE results in a transient amplification of small flow perturbations, even when the dynamics are linearly asymptotically stable.
%
The nonlinearity is energy conserving (i.e.,~lossless) and 
can only redistribute energy between modes~\citep{Sharma2011,WaleffeSIAM1995}.



The interplay between linear and nonlinear terms is 
central transition and turbulence.
%
In many shear flows, laminar-to-turbulent transition can be observed to occur well below the critical Reynolds number $(Re_c)$ determined from a linear stability analysis~\citep{Schmid2001,PatelJFM1969}.
%
This sub-critical transition is partly caused 
by the non-modal growth associated with the linear dynamics~\cite{Trefethen1993,Schmid2001,Schmid2007,ReddyJFM1993}.
%
Indeed, TEG is a necessary condition for transition~\cite{}.
%
Yet, non-modal TEG alone is not 
sufficient to cause transition.
%
While TEG pushes the flow state away from the equilibrium base flow, it is the interaction with the nonlinearity that 
triggers secondary instabilities and drives 
the state outside the basin of attraction.
%
Without the nonlinear terms, the notion of a finite basin of attraction would not make sense.
%
Interestingly, although the nonlinearity is lossless and energy conserving, it interacts with the linear dynamics in such a way as to increase the maximum TEG~(MTEG) that can be achieved~\cite{Kerswell2018}.
%
These transition scenarios cannot be analyzed without accounting for the nonlinear terms in NSE.
%
%


Analysis methods, such as resolvent analysis, have been proposed to account for the interplay between the linear and nonlinear
terms in the analysis of transitional and turbulent flows~\citep{McKeonJFM2010,JovanovicJFM2005}. 
%, passivity ~\citep{Heins2016,Damaren2016,Damaren2018} and dissipation inequality~\citep{Ahmadi2018}.
The resolvent analysis framework leverages the fact that the NSE can be expressed as a feedback interconnection between a linear operator and a nonlinear operator---a so-called Lur'e decomposition.
%
Resolvent analysis goes a step further to consider the nonlinearity 
as an implicit forcing input on the linear dynamics~\citep{McKeonJFM2010,TairaModal2017}.
%
This perspective greatly simplifies the resulting analysis problem, as only the linear system---described by input-output properties of the 
linear resolvent operator---need 
to be analyzed.
%
Within the context of turbulent flows, resolvent analysis provides information on how fluctuations in a time-averaged flow are attenuated or amplified from nonlinear effects.
%
Resolvent analysis has been successfully employed in various contexts~\cite{Taira2019}: identification of coherent structures in wall-turbulence in pipes~\citep{SharmaJFM2013}, identification of triadic nonlinear interaction between resolvent modes~\citep{MckeonAndSharmaPoF2014}, obtaining insights into compressible open cavity flows~\citep{Sun2019}, and passive flow control using riblets~\citep{Chavarin2019}.
%
% The resolvent analysis is 
% an input-output framework that 
% exploits properties of the linear resolvent operator to extract insights about flow physics.
% %
% Within the context of turbulent flows, resolvent analysis provides information on how fluctuations in a time-averaged flow are attenuated or amplified from nonlinear effects. However, the resolvent framework does not explicitly account for the structure of the nonlinearity. %However, it is essential to note the resolvent operators requires only the linear term, the nonlinear term is assumed to implicitly force the resolvent operator to obtain desired output. 

Related methods have been proposed to account for the nonlinearity more directly.
%
% Additionally, the passivity framework~\citep{Khalil} accounts for structure in the nonlinear terms---leveraging the passivity observed in the nonlinearity of the NSE. 
The passivity framework has been shown to be effective in flow control 
based on the nonlinear NSE~\citep{Heins2016,Damaren2016,Damaren2018}. %In~\citep{Heins2016,Damaren2016,Damaren2018}, passivity-based control methods for turbulent flows are proposed.  These methods 
In these studies, the passivity property~\citep{Khalil} of the nonlinear terms in the NSE are leveraged to design linear controller that can stabilize the full Lur\'e system. 
%Here a output feedback controller is developed to force the linear dynamics to be passive, without fully accounting for the exact nonlinearity. 
%In both the resolvent and passivity analysis framework the nonlinear term is not explicitly accounted for.
%
Further advances have been made in input-output methods to study performance, worst-case amplification, stability, and transition for NSE using dissipation inequalities~\citep{Ahmadi2018}. 
% In \citep{Ahmadi2018}, the dissipation inequalities framework is reformulated for the NSE. 
%
Dissipation inequalities derived from NSE can be posed as linear matrix inequality~(LMI) problems, which are then solved using convex optimization methods to successfully analyze various wall-bounded shear flows. 
%
These techniques generalize the classical energy-based analysis approaches~\cite{Schmid2001,josephBook} and also have close ties with nonlinear Lyapunov stability analysis approaches developed for NSE based on sum-of-squares~(SOS) optimization~\cite{goulart2012}.


% Alternatively, a wide range of analysis techniques have been proposed to assess the stability of fluid flows: e.g.,~modal and non-modal stability analysis~\cite{Theofilis2011, Schmid2007,McKeonJFM2010,TairaModal2017,Taira2019,Kerswell2018} as well as more recent undertakings that generalize the classical energy-based analysis approach~\cite{Schmid2001,josephBook} with Lyapunov analysis~\cite{goulart2012}. While the community has made significant progress in stability analysis and prediction, the most reliable of the existing analysis approaches still tend to provide conservative estimates for transition thresholds~\cite{Ahmadi2018}.

%Lur'e decomposition of NSE.  Connections to resolvent/passivity/dissipation inequalities/etc.

%Turbulent flows. Resolvent. Triadic interactions (McKeon, 2017).



In this paper,
we propose a constrained nonlinear systems analysis approach that 
exploits the Lur'e decomposition of NSE to account for nonlinear 
flow interactions with minimal complexity.  
%
The approach is predicated on the fact that nonlinear flow interactions are 
constrained by the physics encoded within the nonlinear terms in the NSE---e.g.,~the nonlinearity is energy conserving and lossless.
%
Mathematically, these physics can be expressed as quadratic constraints between the 
inputs and outputs of the nonlinearity.
%
In turn, these quadratic constraints serve as reduced-complexity models for the nonlinear terms, and can be incorporated within a Lyapunov-based analysis to  perform reliable stability and input-output analysis in the nonlinear setting.
%
The general framework introduced here is applicable to any system that has (non-normal) linear dynamics acting in feedback with a lossless nonlinearity---the NSE being a special case.
%
To establish a proof-of-concept, we formulate and demonstrate the proposed analysis framework on the nonlinear Waleffe-Kim-Hamilton (WKH) model of transition and sustained turbulence~\citep{WaleffeSIAM1995}. 
%

 (move this bit to the WKH model section?).
Similar to the NSE, we first express the WKH system in Lur\'e form---a non-normal linear element in feedback interaction with a static lossless nonlinear element. Here, we formulate several quadratic constraints and investigate the role of the nonlinear terms for stability and transient energy growth analysis within the WKH model. In addition to passivity of the nonlinear term, the nonlinearity in wall-bounded shear flows has a stronger property of being lossless or energy conservation, which can be leveraged. Since the WKH model is developed to mimic the NSE's behavior in shear flows, the nonlinear terms in the WKH model are energy conserving as well. 
 


In Section~\ref{}, we introduce the WKH model in Lur'e form.
%
We then proceed to formulate a global stability analysis problem in Section~\ref{}. We show that the energy-conservation property of the  nonlinearity can be accounted for in the stability analysis via the addition of a quadratic lossless constraint. We find that the lossless constraint alone enables prediction of the critical Reynolds number ($Re_c$) for global instability in the WKH system, and is consistent with the $Re_c$ found by Waleffe using other means~\citep{WaleffePOF1995}.
%
Also in Section~\ref{}, we show that the quadratic constraints framework can be extended to conduct local stability analysis, which is needed when $Re>Re_c$ and the equilibrium point is no longer globally asymptotically stable.
%
This is done by formulating
an additional set of ``local'' quadratic constraints that represent the influence of the nonlinearity when the flow is restricted to a local neighborhood about the equilibrium point.
%
%These ``local'' constraints extend the stability and MTEG analyses to Reynolds numbers beyond the critical Reynolds number for global instability.  
By modifying the size of the local region, the influence of the nonlinearity can be assessed. Given that the linear system is asymptotically stable for all $Re$, we show that the nonlinear term has a destabilizing effect on the system.
%
In Section~\ref{}, we formulate an analysis problem to determine the maximum transient energy growth~(MTEG) that can be realized by a given system.
We shown that the lossless and local constraints increase the MTEG attained in the non-normal and nonlinear WKH system, consistent with findings from nonlinear non-modal stability analysis of NSE~\cite{Kerswell2018}.  Indeed, these findings confirm previous findings~\cite{Kerswell2018} that the optimal disturbance for the nonlinear system is different from the linear optimal disturbance that is often used to study transition.
%
When multiple constraints are included in the analysis, it becomes possible to identify dominant nonlinear flow interactions that underly the dynamics by analyzing the multipliers used to enforce the constraints within the analysis.  In Section~\ref{}, we demonstrate that---without any a priori knowledge---the proposed analysis approach is able to extract the same dominant nonlinear flow interactions whose physical importance is argued in~\citep{WaleffePOF1995,WaleffeSIAM1995}.
%
Finally, we provide concluding remarks of our study in Section~\ref{sec:Conclusion}.
% A coarse outline of the paper follows.
% %
% Section~\ref{} present the WKH model.
% %
% Quadratic constraints for conducting global and local stability analysis are presented in Section~\ref{} along with the results of these analyses.
% %
% Section~\ref{} introduces the MTEG analysis problem and reports results for both global and local MTEG analysis.
% %
% A multiplier-based analysis is conducted in Section~\ref{}, which allows dominant nonlinear flow interactions to be identified.
% %
% Conclusions are drawn in Section~\ref{}.



% The contributions of this work are:
% %\msh{
% %\begin{itemize}
%   % \item Global stability Analysis: 
%  \begin{enumerate}

%     \item This work extends the linear system analysis methods by accounting for the nonlinear terms in the system. The energy conserving nonlinearity in the WKH system is accounted for via the addition of a quadratic lossless constraint. The lossless constraint alone enables prediction of the critical Reynolds number for global instability in the WKH system. This finding is consistent with the findings reported in Waleffe~\citep{WaleffePOF1995}.
%     %\item Local stability Analysis: 
    
%     \item Beyond the global stability regime in the WKH system, the quadratic constraint framework is extended to represent ``local'' nonlinear properties as ``local'' quadratic constraints---for analyzing stability of the nonlinear system in a local neighborhood of a given equilibrium point. These ``local'' constraints extend the stability and MTEG analyses to Reynolds numbers beyond the critical Reynolds number for global instability.  By modifying the size of the local region, the influence of the nonlinearity can be assessed. Given that the linear system is asymptotically stable for all $Re$, we show that the nonlinear term has a destabilizing effect on the system.
    
%     %\item Maximum transient energy growth analysis: 
%     \item Additionally, it is shown that the lossless and local constraints serves to enhance MTEG in the non-normal and nonlinear WKH system, consistent with findings from nonlinear non-modal stability analysis~\cite{Kerswell2018}.  Indeed, these findings confirm that the optimal disturbance for the nonlinear system is different from the linear optimal disturbance that is often used to study transient energy growth and transition.
    
%     %\item Additional constraints can be introduced to constrain the flow state to remain within a local region of the equilibrium point.  These ``local'' constraints extend the stability and TEG analyses to Reynolds numbers beyond the critical Reynolds number for global instability.  By modifying the size of the local region, the influence of the nonlinearity can be assessed.  (state something about the results.)
%     %\item 
%     \item Lastly, when multiple constraints are included in the analysis, it becomes possible to identify dominant nonlinear flow interactions by analyzing the multipliers used to enforce the constraints within the analysis.  It is demonstrated that---without any a priori knowledge---the proposed analysis approach is able to extract the same dominant nonlinear flow interactions whose physical importance is argued in~\citep{WaleffePOF1995,WaleffeSIAM1995}.
% %\end{itemize}
%  \end{enumerate}
%These bullets can be integrated with the paper organization outline below.  This would make it more useful, since it would be a summary of results.  No need to start sentences with ``In Section...", but can ends sentences with ``\dots, as will be shown in Section\dots'' instead.
%}
%\ak{Note to self: try combining contributions and organization into 1 section?}
%
% This paper is organized as follows: Section~\ref{sec:WKH} introduces the fluid flow model used in our analysis. In Section~\ref{sec:QC_stability}, we briefly describe the global property of the nonlinear terms in the WKH model and also introduce the quadratic constraints framework for both global and local stability, while also discussing stability results. In Section~\ref{sec:QC_MTEG}, we formulate quadratic constraints framework for both global and local MTEG analysis.  This sections also discuss the results obtained from local MTEG analysis. In Section~\ref{sec:Lagrange_Mul_Analysis}, we discuss how the quadratic constraint framework can be used to draw physical insights regarding dominating nonlinear flow interactions using Lagrange multiplier analysis. Finally, we provide the concluding remarks of our study in Section~\ref{sec:Conclusion}.
